Adaptive Knowledge-Enhanced Bayesian Meta-Learning for Few-shot Event Detection

Event detection (ED) aims at detecting event trigger words in sentences and classifying them into specific event types. In real-world applications, ED typically does not have sufficient labelled data, thus can be formulated as a few-shot learning problem. To tackle the issue of low sample diversity in few-shot ED, we propose a novel knowledge-based few-shot event detection method which uses a definition-based encoder to introduce external event knowledge as the knowledge prior of event types. Furthermore, as external knowledge typically provides limited and imperfect coverage of event types, we introduce an adaptive knowledge-enhanced Bayesian meta-learning method to dynamically adjust the knowledge prior of event types. Experiments show our method consistently and substantially outperforms a number of baselines by at least 15 absolute F1 points under the same few-shot settings.

==> sec3-method-old.tex <==
\section{Adaptive Knowledge-Enhanced Bayesian Meta-Learning}

\begin{figure*}
    \centering
    \includegraphics[scale=0.2]{fig/over.png}
    \caption{Framework overview. Our method combines both the external knowledge and the support set into a prior distribution of event prototype.  We customize a unified structure to generate sample representations and knowledge representations. Then we utilize the support set to generate a learnable offset for revising the aligned knowledge representations to generate the prior distribution for prototype representations. Finally, we use stochastic gradient Langevin dynamics to draw samples of prototypes for prediction.}
    \label{fig:over}
\end{figure*}


%% 本节将介绍我们提出的知识修正的贝叶斯元学习
\reza{In this section, we present our adaptive knowledge-enhanced few-shot event detection approach.
The overall structure of our method is shown in Figure \ref{fig:over}.
Our method represents each event type with a prototype vector, which is then used to classify the query sentences.
Different from the traditional prototype network, which learns a point estimation of the prototype vectors from the support set, we learn a posterior distribution of each prototype vector through a knowledge-{based} Bayesian meta-learning method.
The posterior distribution is determined by the \emph{knowledge prior} and the \emph{likelihood function} on the support set.
The adaptive knowledge-based prior of prototype vectors is composed of two terms: (i) a prior knowledge vector obtained from the knowledge encoder, 
%which has the same structure as sentence encoder; 
and (ii) a learnable knowledge offset between the prior knowledge and the support set, which results in an \emph{adaptive} knowledge-enhanced prior.
%
By using the adaptive knowledge-based prior, our method can effectively generalize to new event types that cannot be precisely matched in FrameNet.
%
The posterior distribution in Bayesian meta-learning has a complicated form.
So we leverage Monte Carlo sampling to approximate the posterior distribution and draw each prototype sample by the stochastic gradient Langevin dynamics~\cite{welling2011bayesian}.
Our approach can thus be optimized in an end-to-end fashion.
% 
%We first give the problem definition in Section \ref{sec:probdef}.
%Then we introduce the knowledge in \emph{FrameNet} in %Section \ref{sec:knowledge}.
%In Section \ref{sec:encoder}, we present the encoders for the knowledge and sentences.
%We then introduce our knowledge-\reza{based} Bayesian meta-Learning for few-shot event detection in Section \ref{sec:fixbayes}.
In the rest of this section, we explain the framework in more details. 
}
%\subsection{Knowledge-\reza{based} Bayesian Meta-Learning}
%\label{sec:fixbayes}

%After getting the encoding of samples and knowledge, we will use the knowledge-\reza{based} Bayesian meta-learning method to model the posterior distribution of prototype vectors of the event types. 
%The posterior distribution is composed of two terms: (i) a prior of the prototype vector obtained from the event knowledge, and  and (ii) a likelihood function on the support set. 
%
%We first introduce the probabilitstic formalization of Bayesian meta-learning in Section \ref{sec:probform}, and Section \ref{sec:parapost} shows the parameterization of the posterior Distribution. In Section \ref{sec:knowfixed}, we propose the knowledge-adapted posterior distribution. Finally, we introduce the method of optimization and prediction of our method in Section \ref{sec:optpred} and give an intuitive interpretability analysis of knowledge posterior distribution in Section \ref{sec:explain}. 

\subsection{Probabilistic Formalization}
\label{sec:probform}

\reza{Our approach aims to learn the conditional probability distribution $p(Y_Q |X_Q,X_S,Y_S,\mathscr{F})$.  In order to facilitate analysis and calculations, our goal can be stated as computing the following log-probability:}
%
 \begin{equation}
    \label{eq:target}
    \log \ p(Y_Q |X_Q,X_S,Y_S,\mathscr{F})
\end{equation}
\reza{We denote the prototype vector of each event type $t \in T_S$ as $v_t$, which summarizes the semantic meaning of that event type. By introducing the prototype vectors, the log-probability in Eqn~(\ref{eq:target}) can be factorized as:}
%
\begin{equation}
    \label{eq:fac}
    \begin{aligned}
        &\log \ p(Y_Q |X_Q,X_S,Y_S,\mathscr{F}) \\
        =&\log \int p(Y_Q |X_Q,V_{T_S})p(V_{T_S}|X_S,Y_S,\mathscr{F}) \, dV_{T_S}
    \end{aligned}
\end{equation}
%
\reza{where $V_{T_S} = \{ v_t \}_{t\in T_S}$ is the collection of prototype vectors  for all event types in $T_S$. The distribution $p(V_{T_S}|X_S,Y_S,\mathscr{F})$ conditions the probability of prototype vectors on both the support set and event knowledge. 
With the prototype vectors representing the target event types, the distribution of query sample labels can be defined as:
\begin{equation}
    \label{eq:queryprob}
       p(Y_Q |X_Q,V_{T_S}) = \prod_{q \in Q} p(y_q|x_q,V_{T_S})
\end{equation}
where
\begin{equation}
    \label{eq:queryprob1}
       p(y_q = t |x_q,V_{T_S}) = \frac{\exp(\mathcal{E}(x_q) \cdot v_t)}{\sum_{t' \in T_S} \exp(\mathcal{E}(x_q) \cdot v_{t'})} 
\end{equation} 
%
The dot product of the sample encoding $\mathcal{E}(x_q)$ and the prototype vector $v_t$ estimates the similarity between the sample and an event type, and we use a $softmax$ function to normalize the result to get the probability that $x_q$ can have for each event type $t$.
%
%After that, the posterior distribution of prototype vectors conditioned on the support set and the knowledge $p(V_{T_S}|X_S,Y_S,\mathscr{K})$ has not been parameterized. Next we will introduce the parameterization of the posterior distribution.
We next explain our parameterisation of the posterior distribution of prototype vectors given the support set and the knowledge $p(V_{T_S}|X_S,Y_S,\mathscr{F})$.}

\subsection{Adaptive Knowledge-enhanced Posterior Distribution}
\label{sec:parapost}

\reza{
Parameterizing the posterior probability is the key link in our method. The posterior distribution can be factorized into a prior distribution given the event knowledge and a likelihood function on the support set \cite{qu2020few}. Therefore, we formally represent the posterior as follows:
\begin{equation}
    \label{eq:postfac}
       p(V_{T_S} |X_S,Y_S,\mathscr{F}) \propto p(Y_S|X_S,V_{T_S})p(V_{T_S}|\mathscr{F})
\end{equation}
where $p(Y_S|X_S,V_{T_S})$ is the likelihood  on the support set, and $p(V_{T_S}|\mathscr{F})$ is the knowledge-based prior for the prototype vectors.
}

\reza{
Let us assume that we have a vector representation $h_t$ of the knowledge via our knowledge encoder for the event type $t$ (see Section \ref{sec:encoder}). This can reflect the sample characteristics by aggregating the encoding of the knowledge-driven trigger words and the knowledge-driven contextual encoding corresponding to the event type $t$.
%
The vector representation $h_t$ can serve as regularization for the prototype vector $v_t$ through the prior distribution.
%
In practice, we found that not all event types can have an exactly matched frame from \emph{FrameNet}, as the event types have finer granularity.
%
%The reason why the event types cannot exactly match frames is that these event types have finer granularity.
For example, there is no exactly matched frame for the event type \emph{Contact.Online-Chat}, which is a special behavior belonging to the frame \emph{Chatting}.
%
Therefore, it is unreasonable to directly use $h_t$ to construct the prior distribution $p(V_{T_S}|\mathscr{F})$.
%
Tackling the problem of deviations between the knowledge and actual event types is one of the main contributions of our paper through \emph{adaptive} knowledge-based prior, which is explained below.
}

\reza{
Although we cannot find the exactly matched frame for each event type, we can find their super-ordinate frames.
As shown in Figure \ref{fig:example1}, the definitions of an event type and its super-ordinate event type are close.
The super-ordinate frames are also helpful for event detection, so we can use them as the knowledge of an event type.
Thus the knowledge $F_t$ of event type $t$ is from the exactly matched frame or its super-ordinate frame. 
}

\reza{
In order to enable the knowledge-based prior distribution   to accurately reflect the characteristics of the corresponding event type, we add a learnable \emph{knowledge offset} to the prior distribution.
We denote the knowledge offset between the event type $t$ and its knowledge encoding $h_t$ by $\Delta h_t$.
Recall that the knowledge in $h_t$ is encoded from the exactly matched frame or the super-ordinate frame. We  use the follow form to represent $\Delta h_t$:
\begin{equation}
    \label{eq:delt}
    \Delta h_t = \lambda_{t} \odot (m_t - h_t)
\end{equation}
where $m_t$ is the mean value of all sample encodings in the support set which are labeled as event type $t$, and $\odot$ is the element-wise product.
%
The adaptive weight (gate) $\lambda_{t} \in [0,1]^{|h_t|}$ is  obtained by both the sample encoding $m_t$ and the knowledge encoding $h_t$,
\begin{equation}
    \label{eq:lambda}
    \lambda_{t} = \sigma(W_{\lambda}\left[m_t;m_t-h_t;h_t \right] + b_{\lambda} )
\end{equation}
where $\sigma$ is the nonlinear sigmoid  function, 
%that outputs a number between 0 and 1, 
and $W_{\lambda}$ and $b_{\lambda}$ are trainable parameters. The support set mean is defined as,
\begin{equation}
    \label{eq:mean}
    m_t = \frac{\sum_{s \in S, y_s=t} \mathcal{E}(x_s) }{\sum_{s \in S} \boldsymbol{1}(y_s=t)}
\end{equation}
where $\boldsymbol{1}(y_s=t)$ is indicator function, i.e.  $\boldsymbol{1}(y_s=t)$ is one if $y_s=t$, and zero otherwise.
%$\boldsymbol{1}(y_s=t)=0$.
}

\reza{
We aim to fix the knowledge prior through the characteristics of samples corresponding to the event type $t$ in the support set. 
%
This is enabled by our unified architecture that encodes them in the same semantic space. 
%
Furthermore, we note that the samples of an event type $t$ must contain the information needed by $\Delta h_t$. 
%
If there is deviation between event type $t$ and its prior knowledge $F_t$, it indicates that $F_t$ corresponds to the super-ordinate frame of the type $t$ and needs to be further corrected. 
%
We argue that the samples in the support set contain the information needed for the knowledge correction. 
%
If the deviation between samples and $F_t$ is not the deviation between event type $t$ and the frame corresponding to $F_t$, the samples will not be labeled as the event type $t$. This contradicts the assumption, so the support set must contain the deviation between event type and knowledge.
}

\reza{
Putting it altogether, the knowledge prior distribution has the following form,
\begin{equation}
    \label{eq:priorfixed}
       p(V_{T_S} |\mathscr{F}) = \prod_{t \in T_S} p(v_t|h_t,\Delta h_t) = \prod_{t \in T_S} \mathcal{N}(v_t|h_t + \Delta h_t,\boldsymbol{I})
\end{equation}
where $\mathcal{N}(v_t|h_t + \Delta h_t,\boldsymbol{I})$ is a Gaussian distribution with the mean $h_t + \Delta h_t$ and covariance $\boldsymbol{I}$, which is a diagonal matrix whose diagonals are all 1. 
Therefore, each prototype vector has a prior distribution  containing knowledge from \emph{FrameNet}.
%
We can generalize the prior distribution to other event types given new event knowledge.
}


\subsection{Optimization and Prediction}
\label{sec:optpred}

\reza{
During the process of optimization and prediction, we have to maximize or compute the log-probability $\log \ p(Y_Q |X_Q,X_S,Y_S,\mathscr{F})$. However, according to Eqn~(\ref{eq:fac}), the log-probability relies on the integration over prototype vectors, which is difficult to calculate. Therefore, we estimate it with Monte Carlo sampling~\cite{qu2020few},
%
\begin{equation}
    \label{eq:Monte}
    \begin{aligned}
        p(Y_Q |X_Q,X_S,Y_S,\mathscr{F}) 
       & = \mathbb{E}_{ p(V_{T_S}|X_S,Y_S,\mathscr{F}) } \left[ p(Y_Q |X_Q,V_{T_S}) \right] \\
        & \approx  \frac{1}{N_s} \sum_{i=1}^{N_s} p(Y_Q |X_Q,V_{T_S}^{ \left( s \right)})
    \end{aligned}
\end{equation}
%
where $N_s$ is the number of samples, and $V_{T_S}^{ \left( s \right)}$ is a sample drawn from the posterior distribution, i.e.\ $V_{T_S}^{ \left( s \right)} \sim p(V_{T_S}|X_S,Y_S,\mathscr{F}) $. To sample from the posterior, we make use of the stochastic gradient Langevin dynamics~\cite{welling2011bayesian} with multiple stochastic updates. Formally, we can initialize the sample $\hat{V}_{T_S}$ and iteratively update the sample as follows,
%
\begin{equation}
    \label{eq:update}
    \begin{aligned}
        \hat{V}_{T_S} \gets \hat{V}_{T_S} &+ \frac{\epsilon}{2} \nabla_{\hat{V}_{T_S}} log \ p(Y_S|X_S,\hat{V}_{T_S})p(\hat{V}_{T_S}|\mathscr{F}) \\
        &+ \sqrt{\epsilon} \boldsymbol{z}
    \end{aligned}
\end{equation}
%
where $\boldsymbol{z} \sim \mathcal{N}(\boldsymbol{0},\boldsymbol{I})$, and $\epsilon$ is a small real number representing the update step size.
The Langevin dynamics requires a burn-in period.  To speed up the convergence, we follow the previous method \cite{qu2020few} and initialize the sample as follows, 
\begin{equation}
    \label{eq:initialize}
    \begin{aligned}
        \hat{V}_{T_S} &\gets \{ \hat{v}_{t} \}_{t \in T_S} \\
        \hat{v}_{t} &\gets m_t + h_t + \Delta h_t - m
    \end{aligned}
\end{equation}
where $m$ is the mean encoding of all the samples in the support set. Qu et al. \cite{qu2020few} proved in their work that this initialization method can lead to quick convergence of Langevin dynamics.
}

\reza{
After obtaining the samples of prototype vectors from their posterior distribution, $\log \ p(Y_Q |X_Q,X_S,Y_S,\mathscr{F}) $ is approximated according to Eqn~(\ref{eq:Monte}). 
%
During the training stage, we optimise the log-likelihood of query set based on the samples from the posterior constructed using the support set and the knowledge. 
%
In the prediction stage, the log-likelihood will determine the probability that the query sample belongs to each event type. The training process is shown in Algorithm \ref{alg:A}. 
}

% \begin{algorithm}
%     \caption{Training Process}
%     \label{alg:A}
%     \begin{algorithmic}
%         \STATE \textbf{Given:} event type set $T$, event knowledge from \emph{FrameNet} 
%         % 
%         \STATE  \textbf{While} not converge \textbf{do:}
%         % 
%         \STATE  \qquad 1. Sample a subset $T_S$ from $T$ to build a FSL task 
%         % 
%         \STATE  \qquad 2. Sample the disjoint support set and query set for $T_S$
%         % 
%         \STATE  \qquad 3. Compute the knowledge encodings $\{h_t\}_{t \in T_S}$
%         % 
%         \STATE  \qquad 4. Compute the sample encodings $\{m_t\}_{t \in T_S}$
%         % 
%         \STATE  \qquad 5. Compute the knowledge offset $\{\Delta h_t\}_{t \in T_S}$ with Eq. \ref{eq:delt}
%         % 
%         \STATE  \qquad 6. Initialize the prototype vectors $\{V_{T_S}^{s}\}_{s=1}^{N_s}$ with Eq. \ref{eq:initialize}
%         % 
%         \STATE  \qquad 7. Update prototype vectors iteratively with Eq. \ref{eq:update}
%         % 
%         \STATE  \qquad 8. Compute and maximize the log-likelihood function based \\ \qquad on Eq. \ref{eq:Monte}
%         % 
%         \STATE  \textbf{End While}
%     \end{algorithmic}
% \end{algorithm}

\begin{figure}[t]
\small
\removelatexerror
\begin{algorithm}[H]
\caption{Training Process}
\label{alg:A}
%  
\KwIn{Event type set $T$}
\KwIn{Event knowledge from \emph{FrameNet}}

\While {not convergence} {

    Sample a subset $T_S$ from $T$ to build a FSL task 
    
    Sample the disjoint support set and query set for $T_S$
    
    Compute the knowledge encodings $\{h_t\}_{t \in T_S}$ with Eq.~\ref{eq:kencoder}
    
    Compute the sample encodings $\{m_t\}_{t \in T_S}$ with Eq.~\ref{eq:sencoder}
    
    Compute the knowledge offset $\{\Delta h_t\}_{t \in T_S}$ with Eq.~\ref{eq:delt}
    
    Initialize the prototype vectors $\{V_{T_S}^{s}\}_{s=1}^{N_s}$ with Eq.~ \ref{eq:initialize}
    
    Update prototype vectors iteratively with Eq. \ref{eq:update}
    
    Compute and maximize log-likelihood function based on Eq.~\ref{eq:Monte}
}
\end{algorithm}
\end{figure}



\subsection{Intuition  of Adaptive Knowledge-Enhanced Posterior Distribution}
\label{sec:explain}

When knowledge adaption is not used, the form of the prior knowledge distribution of the prototype is as follows,
\begin{equation}
    \label{eq:priorfixed}
       p^o(V_{T_S} |\mathscr{F}) = \prod_{t \in T_S} p^o(v_t|h_t) = \prod_{t \in T_S} \mathcal{N}(v_t|h_t,\boldsymbol{I})
\end{equation}
%
To intuitively show the influence of the knowledge-adapted posterior distribution on the prototype vector, we expand the gradient $\nabla_{\hat{V}_{T_S}} \log \ p(Y_S|X_S,\hat{V}_{T_S})p(\hat{V}_{T_S}|\mathscr{F})$ in eqn \ref{eq:update}. 
The derivation details are shown in the appendix. % \ref{A:GPD}.
For ease of explanation,  we only calculate the gradient of the prototype vector $\hat{v}_{t}$. 
Denote the gradient of the original posterior distribution without knowledge adaption as $g_{\hat{v}_{t}}^o$, and the gradient of the knowledge-adapted posterior distribution as $g_{\hat{v}_{t}}^s$; we get that,
\begin{align}
    \label{eq:go}
    g_{\hat{v}_{t}}^o = &\sum_{s \in S, y_s = t} (1-p_{s}^{(t)})\mathcal{E}(x_s) + C(h_t-\hat{v}_t)\\
% \end{equation}
% \begin{equation}
\label{eq:gs}
        \begin{split}
            g_{\hat{v}_{t}}^s  = &\sum_{s \in S, y_s = t} \left[ (1 - p_{s}^{(t)}) \mathcal{E}(x_s) + \frac{C \lambda_t}{M} \odot \mathcal{E}(x_s) \right] \\ & + C \left( (\mathds{1}-\lambda_t) \odot h_t  - \hat{v}_t \right) 
        \end{split}
    \end{align}
 where $\mathds{1}$ is a $|h_t|$-dimensional vector, and each element of $\mathds{1}$ is 1. $p_{s}^{(t)}=p(y_s|x_s,\hat{V}_{T_S})$ is the probability of correct classification of sample $s$ in the support set and $C=\log \left( 2 \pi \right)^{- \frac{d}{2}} $ is a constant, $d$ is the dimension of prototype (see Appendix A for details). 
%  
 It can be seen that the posterior distribution without knowledge adaption cannot dynamically balance the influence of the knowledge and the support set on the prototype vector, whereas the knowledge-adapted posterior distribution can adjust their contributions to the prototype vector through $\lambda_t$ (see eqn \ref{eq:lambda}). The parameters in eqn \ref{eq:lambda} will be updated by the log-likelihood on the query set. This allows the model to reasonably choose the weight of the knowledge and the support set, and obtain prototype vectors with better generalization. 


\section{Knowledge and Sample Encoder Architectures}
\label{sec:encoder}

\reza{
In this section, we introduce the  architectures of the knowledge encoder and the sample encoder.
The purpose of encoding knowledge is to make up for the lack of diversity and coverage of the support set.
Therefore, the result of knowledge encoding must reflect the true characteristics of the sample space.
%
It is generally the case that the expression of knowledge is more abstract than real samples.
%
For example, ``\emph{Then Jon-O's forces \textbf{ambushed} them on the left flank from a line of low hills.}'' is a real sample of event type \emph{Attack}, whose definition, which is more abstract, is shown in Figure~\ref{fig:example1}.
%
It is important to align the knowledge   and  sample encoding  and map them into the same semantic space.
%
For this purpose, we customize a unified structure for both the knowledge and sample encoder.
}

\reza{
\noindent \textbf{Sample Encoder.} Each sample $x=(I,a)$ is composed of a candidate trigger word $a$ and its context $I$. The context
$I=w_1,\dots,w_l$ is a length-$l$ sentence where $w_j$ is the $j$-th word in $I$, and $a= \left[ b:e \right]$, meaning the candidate trigger word/phrase of $x$ starts at the $b$-th word and ends at the $e$-th word. 
% It can be seen that a specific sample is composed of a candidate trigger word and its context.
We use the candidate trigger word as a query to extract the contextual information related to the trigger. 
First, we use the pretrained language model BERT~\cite{devlin2018bert} to encode the sentence $I$ into a vector sequence $E^x=[e_1^x,…,e_l^x]$, where $e_j^x$ is the encoding vector of the $j$-th word in $I$.
We  denote,
\begin{equation}
    E_a=\frac{\sum_{j \in a} e_j^x}{e-b+1}
\end{equation}
as the encoding of the trigger word.
We then use an attention mechanism to aggregate contextual information. We calculate the query $Q_x$, key $K_x$ and value $V_x$ of the attention mechanism as follows, 
\begin{equation}
    Q_x=f\left(W^Q_x E_a\right); K_x=f\left(W^K_x E^x\right); V_x=f\left(W^V_x E^x\right)
\end{equation}
where $W^Q_x$, $W^K_x$ and $W^V_x$ are the parameter matrices and $f$ is a nonlinear activation function; here we use $tanh$. The encoding vector of the context $E_C$ is,
\begin{equation}
    \begin{aligned}
        E_C &= A^\intercal_x V_x \\
        A_x &= softmax\left(Q^\intercal_x K_x \right)
    \end{aligned}
\end{equation}
where $A^\intercal_x$ is the transpose of $A_x$, and $Q^\intercal_x$ is the transpose of $Q_x$.
}

\reza{
Finally, we concatenate the trigger word encoding $E_a$ and the contextual encoding $E_C$, and use a fully connected neural network to generate the sample encoding vector $\mathcal{E} \left( x \right) $,
\begin{equation}
    \label{eq:sencoder}
    \mathcal{E} \left( x \right) = f \left( W_x^{\mathcal{E}} \left[E_a;E_C \right]+b_x^{\mathcal{E}} \right).
\end{equation}
}

\reza{
\noindent \textbf{knowledge encoder.} Given a knowledge frame $F_t = \{D_t, A_t, L_t\}$ for the event type $t$, 
we encode the frame so that it can reflect the characteristics of real samples.
%
For the knowledge frame $F_t$, the linguistic units $L_t$ can approximately represent the features of the trigger words in the real samples. 
%
Furthermore, the information in the context of the trigger words essentially point to the arguments $A_t$ in the event type's knowledge frame. 
It should be noted that the context information in the sample implies the role information of the event. 
However, directly encoding arguments $A_t$ cannot reflect the role of the arguments in the event.
Thus, we obtain the encoding vectors of $A_t$ in the event by encoding $D_t$, which contains the description of the role of each argument in $A_t$. 
}

\reza{
As shown in Figure \ref{fig:over}, we first add a token $\left[ CLS \right]$ to the beginning of the definition $D_t$ to get $\tilde{D}_t = \left[ CLS \right], d_t^1,\dots,d_t^{l_{D_t}}$, where $l_{D_t}$ is the length of $D_t$ and $d_t^j$ is the $j$-th word of $D_t$.
Then we encode $D_t$ into a vector sequence $E^{\tilde{D}_t} = \left[e^{d_t}_{\left[ CLS \right]},e^{d_t}_1,\dots, e^{d_t}_{l_{D_t}} \right]$. 
In order to use knowledge to construct the characteristics of the sample space, we first construct the knowledge-driven trigger word encoding by aggregating the words in the linguistic unit $L_t$.
The hidden vector $e^{d_t}_{\left[ CLS \right]}$ can represent the meaning of the entire sentence \cite{devlin2018bert}, so we use $e^{d_t}_{\left[ CLS \right]}$ to determine the weight of each word in $L_t$. 
We convert the words in $L_t$ into pre-trained word vectors $E^{L_t} = e^{l_t}_1,\dots,e^{l_t}_{n_{L_t}}$ (here, we use BERT to generate a vector representation of each word), where $e^{l_t}_j$ represent the word vector of the $j$-th word in $L_t$, and $n_{L_t}$ is the number of words in $L_t$. 
Then the knowledge-driven trigger word encoding is calculated as follows:
\begin{equation}
    \begin{aligned}
        E_a^{D_t} &= A^\intercal_{L_t} V_{L_t} \\
        A_{L_t} &= softmax\left(Q^\intercal_{L_t} K_{L_t} \right)
    \end{aligned}
\end{equation}
where
% \begin{equation}
    $Q_{L_t}=f\left(W^Q_L e^{d_t}_{\left[ CLS \right]} \right)$; $K_{L_t}=f\left(W^K_L E^{L_t} \right)$; $V_{L_t}=f\left(W^V_L E^{L_t} \right)$; and 
% \end{equation}
$W^Q_L$, $W^K_L$ and $W^V_L$ are the parameter.
}


\reza{
Similar to the sample encoder, we then need to obtain the knowledge-driven contextual encoding. 
As shown in Figure \ref{fig:example1}, each argument in $A_t$ appears in $D_t$, and after BERT encoding, the hidden vector corresponding to each argument incorporates its semantic information in the event.
So we use the hidden vector of arguments as the knowledge-driven context. We denote the encoding of arguments as $E^{D_t}_{A_t} = e^{A_t}_1,\dots,e_{n_{A_t}}^{A_t}$, where $e^{A_t}_j$ is the encoding vector of the $j$-th argument in $A_t$, and $n_{A_t}$ is the number of arguments in $A_t$. 
An argument may appear multiple times in $D_t$, and we take the mean value of the hidden vectors at different positions as the encoding of the current argument.
Then, we follow the practice of the sample encoder and use an attention mechanism between $E_a^{D_t}$ and  $E^{D_t}_{A_t}$ to obtain the knowledge-driven contextual encoding,
\begin{equation}
    \begin{aligned}
        E_C^{D_t} &= A^\intercal_{D_t} V_{D_t} \\
        A_{D_t} &= softmax\left(Q^\intercal_{D_t} K_{D_t} \right)
    \end{aligned}
\end{equation}
where
% \begin{equation}
    $Q_{D_t}=f\left(W^Q_D E_a^{D_t} \right)$; $K_{D_t}=f\left(W^K_D E^{D_t}_{A_t} \right)$; $V_D=f\left(W^V_D E^{D_t}_{A_t} \right)$; 
% \end{equation}
and $W^Q_D$, $W^K_D$ and $W^V_D$ are the parameter matrices. 
}

\reza{
Finally, we concatenate the knowledge-driven trigger word encoding $E_a^{D_t}$ and the knowledge-driven contextual encoding $E_C^{D_t}$, and use a fully connected neural network to generate the knowledge encoding vector $h_t$ of event type $t$,
\begin{equation}
\label{eq:kencoder}
    h_t = f \left( W_D^{h} \left[E_a^{D_t};E_C^{D_t} \right]+b_D^{h} \right).
\end{equation}
}
